Aggregation of Multiple Knockoffs

We develop an extension of the Knockoff Inference procedure, introduced by Barber and Candes (2015). This new method, called Aggregation of Multiple Knockoffs (AKO), addresses the instability inherent to the random nature of Knockoff-based inference. Specifically, AKO improves both the stability and power compared with the original Knockoff algorithm while still maintaining guarantees for False Discovery Rate control. We provide a new inference procedure, prove its core properties, and demonstrate its benefits in a set of experiments on synthetic and real datasets.

==> Makefile <==
LATEX=pdflatex -synctex=1
LATEXOPT=--shell-escape
NONSTOP=--interaction=nonstopmode

LATEXMK=latexmk
LATEXMKOPT=-pdf -view=none
CONTINUOUS=-pvc

MAIN=ako
SOURCES=$(MAIN).tex Makefile
FIGURES := $(shell find figures/* -type f)
BIB=bibliography

all: once clean

watch: .refresh $(MAIN).pdf

.refresh:
	touch .refresh

$(MAIN).pdf: $(MAIN).tex .refresh $(SOURCES) $(FIGURES)
	$(LATEXMK) $(LATEXMKOPT) $(CONTINUOUS) \
		-pdflatex="$(LATEX) $(LATEXOPT) $(NONSTOP) %O %S" $(MAIN)

force:
	$(LATEXMK) -C $(MAIN)
	touch .refresh
	rm $(MAIN).pdf
	$(LATEXMK) $(LATEXMKOPT) $(CONTINUOUS) \
	    -pdflatex="$(LATEX) $(LATEXOPT) %O %S" $(MAIN)

clean:
	rm -f $(MAIN).pdfsync
	rm -rf *~ *.tmp
	rm -f *.blg *.end *.fls *.log *.out *.brf *.fdb_latexmk \
	*.lof *.toc *.synctex.gz *.synctex.gz\(busy\) *.aux

once:
	$(LATEXMK) $(LATEXMKOPT) -pdflatex="$(LATEX) $(LATEXOPT) %O %S" $(MAIN)

debug:
	$(LATEX) $(LATEXOPT) $(MAIN)


.PHONY: clean force once all watch

